Training Efficient Controllers via Analytic Policy Gradient

Control design for robotic systems is complex and often requires solving an optimization to follow a trajectory accurately. Online optimization approaches like Model Predictive Control (MPC) have been shown to achieve great tracking performance, but require high computing power. Conversely, learning-based offline optimization approaches, such as Reinforcement Learning (RL), allow fast and efficient execution on the robot but hardly match the accuracy of MPC in trajectory tracking tasks. In systems with limited compute, such as aerial vehicles, an accurate controller that is efficient at execution time is imperative. We propose an Analytic Policy Gradient (APG) method to tackle this problem. APG exploits the availability of differentiable simulators by training a controller offline with gradient descent on the tracking error. We address training instabilities that frequently occur with APG through curriculum learning and experiment on a widely used controls benchmark, the CartPole, and two common aerial robots, a quadrotor and a fixed-wing drone. Our proposed method outperforms both model-based and model-free RL methods in terms of tracking error. Concurrently, it achieves similar performance to MPC while requiring more than an order of magnitude less computation time. Our work provides insights into the potential of APG as a promising control method for robotics. To facilitate the exploration of APG, we open-source our code and make it available at https://github.com/lis-epfl/apg_trajectory_tracking.

==> paper-template-latex/chapter/theory.tex <==
\subsection{Theoretical method comparison}

In contrast to the traditional RL setting, we target fixed-horizon problems where a reference trajectory given as $\{\nu_t\},\ \nu_t\in S$ is to be tracked accurately. Thus, we do not maximize a reward, but minimize the Mean Squared Error between states and reference trajectory.
% 
%
We define the task as a discrete time, continuous-valued optimization problem:
\begin{equation}
    \min_{\pi}\\ J^*(\pi) = \mathbb{E}_{\rho(\pi)}  \Big[\sum_{t=0}^{t=T} C(f\big(s_t, \pi(s_t, \nu_{t+1})\big), \nu_{t+1}) \Big],
    \label{eq:prob}
\end{equation}
where $C$ is a cost depending on a given reference state $\nu_{t} \in S$ and the robot state $s_t \in S$; $\rho(\pi)$ is the distribution of possible state-reference pairs  $\lbrace (s_0, \nu_0), \dots, (s_T, \nu_T)\rbrace$ induced by the policy $\pi$. The state at the next time step is given by the dynamics model $f$ with $s_{t+1} = f(s_t, \pi(s_t, \nu)$.
%
The robot state is initialized to the provided reference ($s_0 = \nu_0$). 
%

As typical in the control literature~\cite{borrelli2017predictive}, we define $C$ as the $\ell^p$-norm of the difference between the next state and the reference, together with the control cost, i.e. 
\begin{gather*}
C(f\big(s_t, \pi(s_t, \nu_{t+1})\big), \nu_{t+1}) = 
\\ \Vert  f\big(s_t, \pi(s_t, \nu_{t+1})\big) - \nu_{t+1} \Vert_p + 
 \Vert\pi(s_t, \nu_t)\Vert_p\ .
\end{gather*}
%
For the sake of simplicity, we drop the norm factor $p$ in the rest of the derivation.

We define $\hat{\pi}$ as the optimal controller with dynamics $f$, i.e.,
% In the following, we denote the optimal policy \textit{in the source dynamics $\hat{f}$} by $\pi^*$, which is the policy that minimizes the expected distance from the achieved state from the reference state, formally
\begin{equation} \label{eq:optimal}
    \hat{\pi}(s,v) := \argmin_{\pi} J^*(\pi).
\end{equation}
% It is important to note that the reference $\nu$ might be infeasible for the dynamics $\hat{f}$. %, i.e. unreachable in one time step. 
% Thus, even the optimal controller can be subject to an error $\zeta_{s, \nu}$:
%
% that defines a lower bound on the achievable tracking error, formally
% \begin{equation}\label{eq:zeta}
%   \forall s, \nu\in S \ \ \exists\ \zeta_{s, \nu} \geq 0 :\ \Vert \hat{f}(s, a) - \nu \Vert \leq \zeta_{s, \nu} \ \ \forall a \in A.  
% \end{equation}

\begin{observation} $J^*_{\pi}$ can be optimized directly with respect to $\pi$ via Monte-Carlo estimates of the gradient. This does not require $f$ to be differentiable and enables long-term planning, but requires extensive sampling. This approach is used by both model-free RL~\cite{schulman2017proximal} and some specific instances of model-based RL~\cite{chen2018neural, Heess15svg, hafner2019dream, hafner2019learning}. 
\end{observation}

\begin{observation}
Many model-based RL algorithms~\cite{fu2016one,deng2020soft,bansal2016learning} optimize the nonlinear controller cost in \autoref{eq:prob} online with respect to actions $a$, e.g. via iLQR or MPC.
% via online iterative linearization
% Linear model predictive control (MPC) optimizes the tracking error in $\hat{f}$ by linearizing the dynamics, thereby achieving $\pi_{mpc} = \argmin_{\pi} \Vert \hat{f}_{linear}(s, \pi(s, \nu)) -  \nu \Vert$.
% The achievable performance thus depends on the error due to linearizing.
\end{observation}
One drawback for these methods is that actions are selected through online optimization, which could be both prohibitively slow and difficult to solve for non-convex dynamics depending on high-dimensional observations.

\begin{observation}
Imitation learning methods solve the control task by imitating an expert $\pi_{exp}$ and minimising $\mathbb{E}_{\rho(\pi)}  \Big[\sum_{t=0}^{t=T} \Vert f\big(s_t, \pi(s_t, \nu_{t+1})\big) -  f\big(s_t, \pi_{expert}(s_t, \nu_{t+1})\big)\Vert\Big]$ with gradient descent and data-set aggregation techniques~\cite{ross11a,kaufmann2020RSS,pan2018agile}. These methods therefore minimize an upper bound of $J^*(\pi)$; i.e. their performance is limited by the expert.
\end{observation}
